Part Segmentation for Highly Accurate Deformable Tracking in Occlusions via Fully Convolutional Neural Networks

Successfully tracking the human body is an important perceptual challenge for robots that must work around people. Existing methods fall into two broad categories: geometric tracking and direct pose estimation using machine learning. While recent work has shown direct estimation techniques can be quite powerful, geometric tracking methods using point clouds can provide a very high level of 3D accuracy which is necessary for many robotic applications. However these approaches can have difficulty in clutter when large portions of the subject are occluded. To overcome this limitation, we propose a solution based on fully convolutional neural networks (FCN). We develop an optimized Fast-FCN network architecture for our application which allows us to filter observed point clouds and improve tracking accuracy while maintaining interactive frame rates. We also show that this model can be trained with a limited number of examples and almost no manual labelling by using an existing geometric tracker and data augmentation to automatically generate segmentation maps. We demonstrate the accuracy of our full system by comparing it against an existing geometric tracker, and show significant improvement in these challenging scenarios.

==> related_work_old.tex <==
Generative methods based on geometric calculation fitting template models to observations, which has relatively high accurate comparing to other methods. Also, it has advantages in easily transforming the tracking procedure to other objects. However, lacking semantic classification of input data, most generative methods cannot achieve single frame tracking, which makes them rely on manually initialization and hard to recover from lost tracking frames. \atwnote{I would break the paragraphs between generative and discriminative methods, and include references discussing how these methods work.}  There are also many tracking algorithms proposed in recent years based on discriminative methods which verifying the pose from input data directly. With pose regressions, it is possible to overcome the disadvantages in generative methods, but the detailed surface is hard to be detect through regressions.\par
The basic idea of our approach is based on combining both two categories of tracking method. In recent works, FCNs have shown a great ability in solving semantic segmentation related problems. Works in \cite{bulat2016human,oliveira2016deep,xia2017joint,long2015fully,noh2015learning} show that FCNs are capable in extracting humans from background, which could be used to filter out most interferences for generative tracking methods. In \cite{xia2017joint}, Xia et al. introduced a impressed work combining the task of pose estimation and semantic segmentation via FCNs. However, since the estimation completely depends on the output of the FCNs, it might not be robust when the FCNs are producing less accurate results, which is normal if training on a small dataset or in the case of occlusions. In our approach, by combining generative methods, the pose tracking would not be interfered by false predictions outside the searching area of pose optimization, allowing our method to be robust to reasonable noises of FCNs. \par
In \cite{ronneberger2015u}, Ronneberger et al. proposed U-Net, an accurate FCN structure. U-Net\cite{ronneberger2015u} has been shown to be extremely accurate in semantic segmentation tasks and can be trained with limited examples. However, due to the complexity of the network, U-Net might not be suitable for real-time tracking task. In our case, rather than just using RGB data as most related works, we have spatial information which allowing us achieve an accurate result by using a simplified FCN architecture. So we proposed a new Fast-FCN structure based on \cite{ronneberger2015u} to keep our tracking system performing in real time.
\atwnote{It's good to talk about how our system works in relation to others here (which you are doing in the last paragraph here), but I think we need more references and more explanation of how existing methods work.  I can pitch in here too.}\wwnote{I modified the part for FCN to be more specific. Hopefully it is looking better now. But I don't have a good background for the discriminative and generative methods. Do you mind help me in this part?}
\atwnote{Yeah, no problem, I will come back in here and add more on that.}
